Bias and Generalization in Deep Generative Models: An Empirical Study

In high dimensional settings, density estimation algorithms rely crucially on their inductive bias. Despite recent empirical success, the inductive bias of deep generative models is not well understood. In this paper we propose a framework to systematically investigate bias and generalization in deep generative models of images. Inspired by experimental methods from cognitive psychology, we probe each learning algorithm with carefully designed training datasets to characterize when and how existing models generate novel attributes and their combinations. We identify similarities to human psychology and verify that these patterns are consistent across commonly used models and architectures.

==> capacity.tex <==
\section{Memorization Capacity Experiments}
We generate a dataset of random noise $\Dc = (x_1, \cdots, x_n) \sim \mathcal{N}(0, I)$. Let $z \to x$ be a generative model, $x \to z$ be an encoder, and $x \to \mathbb{R}$ be a discriminator. Train the following models
\begin{enumerate}
\item A mapping where each $z$ maps to a $x$ in the dataset, preasigned.
\item A mapping from $x$ to the assigned $z$.
\item A VAE on $x$ without pre-assignment of $(x, z)$.
\item A GAN on $\Dc$.
\item A Discriminator between the resulting samples from the GAN and $\Dc$.
\end{enumerate}
To measure how much the generated samples is identical to the random noise, we compute the nearest neighbor. For each sample not in the dataset, the expected distance between nearest neighbor should be $x - x' \sim \mathcal{N}(0, 2I)$, so the probability that $E[\lVert x - x' \rVert_2^2] = 2d$ with tight concentration bounds. 

Expected observation: 1 and 2 are successfully learned. 3 is possibly learned, 4 is not learned, 5 can discriminate. 

Idea: compare with 1 generator train vs k discriminator train. If the lack of memorization comes from iterative procedure, then should observe that larger k leads to better memorization. 

Current observations: 1 can memorize a images of size $[28, 28, 1]$ for about 4000 examples, more examples has not been tested. VAE seems to be unable to even memorize 100, and GANs cannot memorize at all. Other sizes are to be tested. A hypothesis is that VAE sinks into local minimum or very flat saddle points and cannot differentiate z for different value of x. There do exist a solution (separately trained encoder and decoder) that memorizes, though this remains to be verified. 

% \subsection{Two Models for the Random Noise Experiment}
\begin{table}
\begin{tabular}{ccc}
& Pro & Con \\ \hline \\ 
Continuous $z$ & \begin{minipage}{0.45\linewidth}
Less likely to suffer from local minimums. 
\end{minipage} & \begin{minipage}{0.45\linewidth}
If partition the measure of $p(z)$ into equal divisions and map each of them to an output, the variational posterior is disjoint, and cannot be represented by a traditional family. 
\end{minipage} \\ \hline \\ 
Discrete $z$ & 
\begin{minipage}{0.45\linewidth}
Can leave out the posterior regularization term because autoencoder is well behaved and $q(z)$ can never have infinite entropy. 
\end{minipage} & 
\begin{minipage}{0.45\linewidth}
Tricky to train and implement. The Gumbel trick in the experiments are unstable. 
\end{minipage} \\ \hline \\
Continuous $x$ &
\begin{minipage}{0.45\linewidth}

\end{minipage} & 
\begin{minipage}{0.45\linewidth}
Must define fairly arbitrary distributions (e.g. fixed variance Gaussian) and unstable (e.g. infinite likelihoods when variance $\to 0$.)
\end{minipage} \\ \hline \\ 
Discrete $x$ & 
\begin{minipage}{0.45\linewidth}
The log likelihood is a natural measure of fit to both training and test set
\end{minipage} & 
\begin{minipage}{0.45\linewidth}
GAN training on discrete input is harder and less common. 
\end{minipage}
\\
\end{tabular}
\caption{Comparison of Experimental Settings for the Noise Experiment}
\end{table}

Another option other than considered in the table is to try an autoencoder where both $x$ and $z$ are continuous. Find the optimal solution to the ELBO manually. 


For VAE model with an additional regularization term, which classifies the image into 500 preassigned labels, it first maps image $x$ to $\left[z_{1}, z_{2}\right]$, where $z_{1}$ is a one hot array with 500 dimensions, trained by cross entropy loss; $z_{2}$ is the standard gaussian distribution. We test the model by generating 500 big images, each belongs to one class, i.e. fixing the label term $z_{1}$ and sampling from the standard gaussian as $z_{2}$.  Each big images contain 64 small images. Around \textbf{80\%} (a little disappointing) are correct. The worst images are shown below.

\begin{figure*}[h]
\centering
\subfigure[]{\includegraphics[width=.45\textwidth]{infoVAE/0419}}
~
\subfigure[]{\includegraphics[width=.45\textwidth]{infoVAE/0471}}
~
\subfigure[]{\includegraphics[width=.45\textwidth]{infoVAE/0473}}
~
\subfigure[]{\includegraphics[width=.45\textwidth]{infoVAE/0481}}

\caption{example fail case for infoVAE model}
\label{fail}
\end{figure*}

\subsection{Storyline}
\begin{enumerate}
\item Discuss generalization and memorization, and why memorization is important (e.g. some combinations are quite arbitrary, apples are never purple and eggplants are never red) \hr{And define the hierarchy of generalization/memorization. e.g., lower generalization means like shape variations (we could borrow something from the icml'17 paper perhaps?), higher generalization means different configurations (type, identity, color, etc.)}
\item GAN/VAEs have memorization issues on modeling a single domain of variables $x$: Use three datasets 1. random noise 2. digit combination 3. object properties \hr{4. structured data, say some Arithmetic sequences and Isobaric sequence}. The first two can be quantitatively measured while the third can be qualitatively evaluated. 
\item GAN/VAEs have memorization issues on two domains $x, y$. Consider conditional maps $y|x$ and joint maps $x, y$\hr{Are there any previous work on joint mapping?}. Show that BiGAN/ALI do not memorize not because of ambiguity (ALICE) and even when MI is maximized they still perform poor inference.
\item \hr{Probable fixes, like additional regularization or batch size/learning rate} 
\end{enumerate}
Question: What is the distinction between one group of variables and two groups? Are they both modeling some joint distribution? What is the relationship between memorization of special configurations and general image modeling. For example, why aren't two ways to draw the number 9 two special configurations?  \hr{We may want to avoid this statement? Just focus on different configurations come from different digits. It seems that at least the first two experiments (random noise and digit) will not lead reviewers to that question easily. Also, it is kinda common sense that '9's (or other digits) have to be similar enough in the dataset, otherwise humankind will not even recognize it?}
Question: How to distinguish from existing work on mode missing?
\hr{We could probably show them that all (or most) modes will be generated as long as they appear in the dataset (true for infovae). Those configurations that are not in the dataset will not necessarily be generated, which is not the definition of mode missing, right?}

Advice from Rui: focus more on natural language datasets to emphasize the importance of memorization. For example, to generate grammatically correct sentences there are at least a few hundred special combinations to remember. Use this as motivation before showing that GAN/VAE cannot memorize. Also focus more on why these models do not memorize. 

Idea: use the bottleneck behavior of $\beta$-VAE to explore the compression a VAE finds. e.g. on similarity based or not similarity based datasets, see if VAE finds the right structure in an effort to compress the training data. Relate to Bayesian neural networks. 


==> old.tex <==
% \subsection{Difference from Statistical Learning Theory}
% We argue in this section that a notion of generalization beyond SLT (e.g. log likelihood on test set) is needed to better understand generative models. 



% There seem to be three distinct settings where generalization is differently defined
% \textbf{1)} Large i.i.d. dataset setting: Assume we have a dataset with size $\propto \log(1/\delta) + \log \lvert \mathcal{H} \rvert$, then high confidence bounds can be provided. In this setting the dataset is always drawn i.i.d. w.r.t. true distribution $p^*$, and our goal is to learn a model such that minimize loss on the training data, while still having some guarantees on the loss on $p^*$. 

% \textbf{2)} Small i.i.d. dataset setting: Assume we have a dataset significantly smaller than required for any SLT to apply. For example, given a single example of an object, what other objects belong to that class. Or another example, given a yellow circle, can we name it $C$, then what does $C$ actually refer to? The yellow color, or the circle? Given more data we will be able to eliminate incorrect hypothesis and obtain SLT generalization bounds, but given one data it seems that truth is entirely subjective, and one must take a subjective Bayesian approach. There is no objective "correctness" to be asserted. 

% An example is the shape bias of human. Humans would associate the name with the circle rather than the color. This is also illustrated by Quine's Inscrutability of reference~\citep{quine2013word}. 

% \textbf{3)} Biased dataset setting: In this case the dataset can be large or small, but we can no longer assume that the training data to be drawn i.i.d. from the ground truth distribution. In fact, the ground truth distribution might not even exist. For example, the digits most people see always follow specific (despite diverse) types of styles. But when presented with digits with exotic styles (e.g. in artistic style), people would still identify the digit as valid and recognizable. Because it is practically impossible to draw samples i.i.d. from the space of ``all recognizable digit images'', some form of generation beyond predictions of SLT must be at work here. As another example, people often recognize the biased-ness of their own experience: there are events that should have very low probability if we assume that observations are i.i.d. but people often assign a much higher probability to these exotic events than the i.i.d. assumption would predict. (Hopefully a psychological experiment here). 

% Therefore to truly understand the generalization of generative models, we must resort to human judgment. We ask two questions: are all the novel samples generated approved by humans, and are all human imagined novel samples assigned high probability by the generative model. 

% \subsection{Alternative Formulation}
% SLT assumes that dataset is drawn i.i.d. from a true distribution. However, this makes three assumptions, each of which can be problematic for generative models

% \textbf{1)} True distribution: the existence of a true distribution is unclear (e.g. what is the set of ``all reasonable looking digits''.) This is in contrast to classification where humans often do have consensus on the classification of an object, and this information can be effectively collected.

% \textbf{2)} i.i.d.: as in previous problem of bias. Something more related to our experiments: humans know their ``effective number of observations''. i.e. even though everyone multiple observations that the earth has one moon, but they would not generalize this conclusion to all planets, because in that case, they only have one observation (despite multiple variants of that same observation).

% \textbf{3)} Large dataset: as in previous problem formulation.

% Difference between generative models and classification: for the latter it's an n-class classification task, that we only evaluate on the support set. for the former it's a two class classification task, but we only have labeled data for one class, and we evaluate on all possible inputs. This makes the three problems more evident (but why?).

% After discussion with Stefano: frame this as whether we would like to learn the true distribution (e.g. 500 digits) vs. the human biased modeling of the distribution (e.g. all 1000 digits). For a model to perform well it must carry inductive bias, so that even given infinite data, there should be distributions that it cannot model. So do humans. 

% Examples:
% Humans should also be very bad at memorizing exceptions. Experiment: given a set of objects with one config missing, ask a human to identify whether that object appeared (memorization experiment).

\section{Old Draft: Memorization vs. Generalization}
Goal: investigate whether a model chooses to memorize random information or generalize, similar to how a human would choose to memorize or generalize (e.g. given a list, a new example in list?)

We also observe empirically that GANs have a surprisingly small memorization capacity, and start to generalize when given only a small number of label combinations during training (as opposed to just 'memorizing' these cases). This is surprising since from the observations in \cite{zhang2016understanding}, a feed-forward neural network can memorize a huge number of random label combinations.
%\shengjia{end intro}

%\js{discuss GAN success, problems with missing modes}
%Generative adversarial networks (GANs,~\cite{goodfellow2014generative}) have achieved huge success in a variety of applications, including image generation~\cite{radford2015unsupervised}, style transfer~\cite{zhu2017unpaired}, and semi-supervised learning~\cite{odena2016semi}. Despite its empirical successes, it has been empirically observed that the superior sample quality of GANs might come at the cost of missing modes.

% However, the likelihood-free approach of GANs make it difficult to quantitatively evaluate the performance and identify issues, such as the ``missing mode'' problem. 
% %\js{modify following for discussion on evaluation; currently copied from Arora's paper} 
% Several approaches have been proposed to address these problems. The Inception score~\cite{salimans2016improved} is proposed as a method to evaluate GAN performance through another powerful pretrained network.
% \cite{wu2016quantitative} propose to measure the log-likelihoods of GANs through Annealed Importance Sampling, transforming the quantitative measure of GANs back to likelihood-based methods. A method to trade-off between sample quality and sample diversity is proposed in \cite{poole2016improved}.

% In this work, we consider evaluating GANs on datasets with special properties -- that it is able to obtain labels from the generated samples. This allows us to use labels as a proxy to analyze the distributions of generated samples and provide a more holistic view than a single numerical metric. Moreover, we reason about the label distributions though Minimum Description Length and draw a connection between the complexity of the label distributions and the minimum encoding length under a certain language. We empirically show that the encoding length of the distribution is strongly correlated with GAN's ability to learn it, and how would GAN generalize when it does not have enough capacity to learn the distribution. This reveals several interesting results, including one that shows GANs does not necessarily perform worse when there are more modes.

% \js{another notion of generalization of deep networks - does GANs generalize?}
% \js{labels as a proxy to analyze distributions; interestingly, when the labels are hard to encode, GAN fails to learn them} \js{not necessarily because of many modes.}

%\subsection{Evaluating Generative Models using Their 

% The downside of this approach, however, is that we ignore the distribution for properties within a single label; the generator can potentially generate a particular sample for some label with high frequency and not be distinguished from a distribution with a large variety of labels with the same label. We assume that this will occur less frequently than the distributional mismatch on the label level, since empirical evidences (such as \cite{radford2015unsupervised}) have suggested that GANs are able to produce similar yet diverse examples by traversing the latent code manifold.

% In the following sections, we show some empirical results on GAN's ability to learn datasets with some random set of labels. We discover an interesting phenomenon: 
% \textit{having more modes does not necessarily hinder GAN's ability to learn the distribution.}

% Based on these observations, we propose a theory based on Minimal Description Length and explain the empirical results with the theory.

\subsection{Learning to Generate Random Labels}
\label{sec:exp}
% \js{another tentative title: do gans always miss modes?}



%\subsection{Evaluating Generative Models using Their Label Distributions as Summary Statistics}



%\subsection{Synthetic Dataset Creation}

We consider a family of distributions where each sample from the distribution is a $56 \times 56$ image that contains three MNIST digits at fixed locations in the image (top left, top right, bottom left, $28 \times 28$ each). Hence, there are a total of $10^3 = 1000$ \textit{combinations}, e.g., `7,1,7' or `9,1,3'. %We use $X_1$, $X_2$ and $X_3$ to denote the individual labels of the three digits respectively.

\textbf{Training Data Generation:} We select randomly a subset of these $1000$ combinations, specifically, 1\%, 4\%, 16\%, 32\%, 50\%, 84\%, 96\%, 99\% of the combinations. We call these sets of combinations $C_1, C_4, \cdots, C_{999} \subseteq \{0,\cdots,9\}^3$. We define $p$ as the ``true combination distribution'', which assigns equal probability to the selected combinations. %\s{define $p$ up here} 
For example, if we select two combinations $(7, 1, 7)$ and $(9, 1, 3)$, then $p(7, 1, 7) = p(9, 1, 3) = 0.5$.
For each $C_i$, we construct a training dataset of images with three digits each, only allowing digit combinations that are in $C_i$, combining individual images of digits from MNIST. We denote the datasets as Rand1\%, Rand4\%, \dots , Rand99\% respectively.
%The distribution of the 10 digits on each location is set to be uniform\s{this doesn't make sense}. 
Each dataset contains 200,000 images in total, and we investigate the distribution of samples from the generative models trained on Rand1\%, Rand4\%, \dots , Rand99\% respectively~\footnote{Training details in Appendix \ref{sec:train}.}. 


\textbf{Evaluating Generative Models using Their Label Distributions as Summary Statistics:}
% We consider the case where the samples are composed of digits with certain high-level properties, such as digit identity and style information.
We propose to focus on high-level properties -- labels in particular -- of the learned generative model distribution. If the generated distribution and the real data distribution are to match, one necessary condition is that the \emph{combinations} of the two distributions should be identical. Moreover, by leveraging digit classifiers with state-of-the-art performance, it is straightforward to obtain the labels of every generated sample with high confidence. This analysis also allows us to visualize the label distribution of the samples and compare with the real distribution and immediately identify whether the generated distributions exhibit certain pathological properties such as mode collapse~\cite{goodfellow2016nips}. Similar approaches have been adopted in \cite{song2017generative,song2017nice} where labels are used to approximately demonstrate mixing of Markov chains.

%\textbf{Training:} We train a GAN on each of these training datasets. \s{Expand}

\textbf{Computing the combination distribution:} We split the generated samples into three $28\times28$ images. The three images are then classified by a pretrained 10-way MNIST classifier $C$ with $<1\%$ error, resulting in one prediction for each image. Then we combine the three prediction to obtain $1$ of the $1000$ combinations as the combined-label for the generated image.
% \s{explain what the classifier predicts. this is extremely confusing because you use labels to mean different things}
% \s{we generate samples from the trained gan. we classify them with $C$. we get an histogram}
This allows us to obtain a histogram for the $1000$ combinations through an empirical estimate. Ideally, the generated combination distribution (denoted $q$) should match the true combination distribution $p$, which has probability $1/\ell$ over the $\ell$ selected combinations $C_i$, and zero probability over others. 
%\s{give an example}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{img/hist}
\caption{Illustration for the experiment in Section \ref{sec:exp}.}
\end{figure}

\textbf{Evaluating the combination distribution:} We consider three methods to compare the distances between $q$ and $p$. Cross entropy (CE) evaluates the average number of bits needed to identify an event in $p$ using coding scheme optimized for $q$; Earth Mover's Distance (EMD) measures the minimum transport from $q$ to $p$. These two methods provide a holistic view about the ``distance'' between $p$ and $q$, yet they do not distinguish errors from assigning the wrong probabilities to the true labels and errors from assigning probability to false labels. Therefore, we propose another performance measure that draws insights from the Area Under the ROC Curve (AUC).

% Area Under the ROC Curve (AUC) \hr{measures the probability that a random positive sample has higher scores than a random negative sample. It }considers the rank of the histogram values and is independent of the specific threshold / class distribution, but does not consider different probability values under the same rank. \s{explain what AUC is. this is not the standard one and is going to be very confusing}

%\s{rephrase, still unclear what this is} 
Consider a classification problem over the combinations $C_i$ where the goal is to distinguish whether some combination is in the support of $p$. Therefore the ground truth label for $C_i$ is $\mathbb{I}(p(C_i) > 0)$. We treat $q(C_i)$ as predictions from the classifier; if $q(C_i)$ is higher, then $C_i$ is more likely to be predicted as positive according to $q$. The ROC curve plots the true positive rate against the false positive rate at various threshold settings; AUC simply measures the area under this curve which considers the rank of the $q(C_i)$ values. This has the advantage of being independent of the specific threshold / portion of selected combinations.
%, but does not consider different probability values under the same rank.
% According to our assumptions, the optimal encoding scheme would ``memorize'' all the labels when the number of labels are small, and try to memorize the exceptions when the number of labels are large. However, since \textit{all} and \textit{except} takes longer coding lengths than \textit{add}, they are considered harder to learn. Thus a dataset with only $1\%$ of the labels should be easier to learn than one with $99\%$ of the labels.


\begin{table}
\centering
\begin{tabular}{c|cccccccc}
\toprule
\% of combinations & 1 & 4 & 16 & 32 & 50 & 84 & 96 & 99 \\\midrule
CE & 0.217 & 0.363 & 0.683 & 1.10 & 0.98 & 0.39 & 0.33 & 0.30 \\
EMD & 0.147 & 0.211 & 0.336 & 0.283 & 0.201 & 0.130 & 0.128 & 0.121 \\
\midrule
AUC & 1.000 & 1.000 & 0.987 & 0.601 & 0.543 & 0.551 & 0.565 & 0.611 \\
\midrule
\midrule
$L(\cdot)$ & 10 & 40 & 160 & 320 & 500 & 193 & 73 & 43 \\
\bottomrule
\end{tabular}
\vspace{1em}
\caption{\textbf{Upper:} Performance measures for the generated distribution when trained on datasets with different portions of randomly preselected combinations. For CE and EMD, lower is better. For AUC, higher is better. \textbf{Lower}: The predicted code length $L(\cdot)$ proposed in Section \ref{sec:theory}, where $c = 10, d = 1$.}
\label{tab:auc}
\end{table}

% In order to make a fair and quantitative comparison between the performance of generative models trained on different datasets, we consider the AUC score~\citep{bradley1997use}, which is a widely used metric to evaluate the performance of classifiers and is independent of the portion of positive/negative labels. 
% Since we are able to evaluate the probability of each label from the distribution of generated samples, we are able to evaluate the ``confidence'' of the generative model that a label belongs to the true distribution -- labels with higher probability in the generated samples are more likely to occur in the true distribution as suggested by the generative model. Hence, we treat the evaluation of a generative model as the evaluation of a classifier that outputs real values for each label. AUC values range from $0$ to $1$: a score of $1$ is perfect, a score of $0.5$ suggests that the prediction is no better than a random classifier, and a score less than $0.5$ means that the classifier is worse than randomly guessing the labels. Therefore, a higher AUC score would suggest that the generator has learned the distribution better, and we use this metric to compare the quality of the generated distribution learned under different datasets.

Table \ref{tab:auc} contains the chosen measures of distances between $q$ and $p$, over training sets with a growing number of digits combinations (modes)~\footnote{We show more detailed figures in the Appendix.}. 
Increasing the number of combinations in the training set,
% initially decreases performance\s{never use a generic word like performance. be as specific as possible}: 
as the number of combinations grows from 1\% to 32\%, CE and EMD increase while AUC decreases (with the exception of EMD at 32\%). This difference in $p$ and $q$ indicates that the generator is either 1) not producing some combinations that were present in the training set (mode collapse) or 2) producing samples with digit combinations that were not present in the training set $C_i$ it was trained on.
%This seems to indicate GANs gradually failing to memorize the data and suffering from mode collapse. 
However, the opposite occurs when the portion of combinations is large: increasing the portion of combinations from 50\% to 99\% actually decreases CE and EMD, while increasing AUC. In this case, \emph{it appears that the model actually performs better with more combinations (modes) in the true distribution!}
%\s{expand this is the key poiny. performance is too generic. give examples from the table. they key point of the paper is summarized in 4 lines. this seems highly suboptimal}

This behavior is unexpected in two ways. On the one hand, it has been shown that neural networks are able to overfit to (or memorize) random labels in supervised learning, yet in the case of GANs, the generated distribution seems to generalize to certain combinations that it has not discovered. On the other hand, it seems that GANs does not always perform worse when there are more combinations/modes in the true distribution, which is contrary to the common belief that GANs would perform worse when there are more modes.
% the model achieves a much worse AUC even when the portion of exceptions is small. This suggests that it might be much harder for the model to learn ``exceptions'' than learn ``enumerations''. What is also surprising is that the model actually performs better when there are more labels in this case; this seems to be in contrast to the common conception that GANs tend to miss modes when the model does not enough capacity. 
While this cannot be simply explained by the ``missing modes phenomenon'', some of these empirical results can be explained by our following theory based on Minimal Description Length. Intuitively, if the distribution is harder to encode, it is harder for GANs to learn that distribution. As a consequence, GAN will learn an imperfect distribution, covering either more or less combinations than what was present in the training set.
%that it could represent using the coding length that it is provided with. 


\section{Measuring the Complexity of Label Distributions}
\label{sec:theory}

The Minimum Description Length (MDL, \cite{rissanen1978modeling}) framework provides a principled way to measure the complexity of the data/distribution. Under a set of allowed codes, there exists a computable minimum encoding length for the data. The minimum encoding length can then be utilized to determine the complexity of the distribution in question.
Natural distributions are generally hard to encode and interpret in terms of Minimal Description Length because it is unclear as to what computer language / symbols should be used in order to represent the distributions. However, this can be made easier for the case of label distributions in our case. %Assume some distribution where each sample contains 3 digits, which results in $10^3 = 1000$ potential configurations. 
To further simplify things, we assume that all the labels within the support of the distribution are equally distributed. That is, for some label distribution $p$: $
p(\ell) = 1 / |\mathrm{supp}(p)|, \forall \ell \in \mathrm{supp}(p)$.

Thus we reduce the problem of describing the distribution $p$ to describing its support set $\mathrm{supp}(p)$. 
We denote $\mathcal{S}$ as the support set with elements $(X_1, \ldots, X_N)$, where $X_i \in \mathcal{X}_i, \forall i \in \{1, \ldots, N\}$. 
Let $L(\cdot)$ denote the minimum code length for any set.
We then assume one particular encoding scheme that is intuitive and satisfies the following conditions:
\begin{itemize}
\item $\forall X_i, L(\{X_i\}) = 1$ (\textit{one})
\item $\forall i, L(\mathcal{X}_i) = c$ for some constant $1 < c < |\mathcal{X}_i|$; (\textit{all})
\item $\forall \mathcal{S}_1, \mathcal{S}_2 \in \mathcal{S}$, $L(S_1 \cup S_2) \leq L(S_1) + L(S_2)$ (\textit{and})
\item $\forall \mathcal{S}_1 \in \mathcal{S}$, $L(\mathcal{S} \setminus \mathcal{S}_1) \leq L(\mathcal{S}) + d L(\mathcal{S}_1) + 1$ for some constant $d \geq 1$ (\textit{except})
\item $\forall \mathcal{S}_i \in \mathcal{X}_i, \mathcal{S}_j \in \mathcal{X}_j$, $L(\mathcal{S}_i \times \mathcal{S}_j) \leq L(\mathcal{S}_i) + L(\mathcal{S}_j) + 1$ (\textit{product}). 
\end{itemize}

Given a fixed model/encoding scheme, the code length of some set/distribution only depends on the set itself. According to this encoding scheme, we are able to intuitively identify several sets/distributions that are ``easy'' or ``hard'' to represent:
\begin{itemize}
\item A distribution with a few possible labels is easy to represent because it is possible to enumerate all the possible labels through \textit{and} with a short code.
\item A distribution with all but few labels should also be easy to represent, since it is possible for the program to represent with the \textit{all} set and enumerate for all the exceptions through \textit{except}.
\item A distribution with a large number of random labels is hard to encode using the encoding scheme described.
% \item A distribution with $n$ labels is easier to represent than one with all but $n$ labels, since \textit{all} and \textit{except} takes longer codes than \textit{and}.
\end{itemize}

So far, we have defined a model that allows us to evaluate the code length required to represent a distribution. In the case considered in this paper, $N = 3$ (digits per image) and $|\mathcal{X}_i| = 10$. And thus we are able to describe the code length for the random label distributions. Assuming $\mathcal{S}$ is some set of $g\%$ random labels
\begin{itemize}
\item From the \textit{and} operation, we have $L(\mathcal{S}) \leq 10 g$;
\item From the \textit{all} and \textit{product} operations, we have $L(\mathcal{X}_1 \times \mathcal{X}_2 \times \mathcal{X}_3) \leq 2 + 3c$;
\item From the \textit{except} operation, we have $L(\mathcal{S}) \leq 3 + 3c + 100 d (10-g)$;
\item Therefore, $L(\mathcal{S}) \approx \min(10g, 3 + 3c + 10 d(100-g))$ and $L(\mathcal{S})$ takes its maximum when 
$$
g^\star = (3 + 3c + 1000d)/(10 + 10d)
$$
%which we denote as $g^\star$.
\end{itemize}

%\s{i dont' think the connection with the experiments comes through. add L to the table? show that it is correlated somehow? }
%\s{never use performance. be specific}
In fact, the minimal code length $L(\cdot)$ of the distribution is closely related to the empirical observations (see Table \ref{tab:auc}), which we relate to GAN's capability of learning it. When $g \leq g^\star$, the \textit{and} operation would be used to encode the distribution; the distribution gets harder to encode with more labels, leading to worse performance in most cases (with the exception of 32 in EMD and 50 in CE). When $g \geq g^\star$, the \textit{all} but \textit{except} case is more dominant, the distribution is easier to encode, so the performance actually gets higher with more labels present. %Moreover, encoding $g\%$ of the labels when $g < 50$ is easier than encoding $(100-g)\%$ of the labels, since encoding \textit{all} and \textit{except} is more expensive than \textit{and}. 
Hence, this MDL perspective would explain the surprising empirical phenomenons that we observe in Section 3. It also tells us how the generative model will generalize when it cannot encode the distributions with many labels -- it will first attempt to encode the \textit{all} case and then the individual \textit{exceptions}. In fact, Figure \ref{Num32} (in the Appendix) shows that the label distributions learned with $50\% - 99\%$ labels are very similar even when trained with a different set of labels.

%In the next section, we will demonstrate empirically that the complexity of the distribution (code length) is closely related to the ability to fit the distribution with GANs. This would suggest that if GANs have limited model capacity, it would ``generalize'' to the distribution to which the encoding scheme would represent within its coding capacity.

% \section{Experiments}

% \subsection{The Three Digits Dataset}
% We consider a family of distributions where each sample from the distribution is a $56 \times 56$ image that contains three digits on fixed locations in the image respectively (top left, top right, bottom left, $28 \times 28$ each). Hence, there are a total of $10^3 = 1000$ available label configurations to choose from. We use $X_1$, $X_2$ and $X_3$ to denote the labels of the three digits respectively.

% \subsection{Learning to Encode Random Labels}
% First, we consider the case where the possible labels are selected randomly from the $1000$ combinations, specifically, 1\%, 4\%, 16\%, 32\%, 50\%, 84\%, 96\%, 99\% of the combinations. We build up datasets with the images whose labels are contained within the set of randomly selected labels. We denote the datasets as Rand1\%, Rand4\%, \dots , Rand99\% respectively.

% The distribution of the 10 digits on each location is set to be uniform. Each subset contains 200,000 images in total, and we investigate the distribution of samples from the generative models trained on Rand1\%, Rand4\%, \dots , Rand99\% respectively. We pretrain a classifier with $<1\%$ error on which we rely during testing to evaluate the combination of the generated samples. 

% According to our assumptions, the optimal encoding scheme would ``memorize'' all the labels when the number of labels are small, and try to memorize the exceptions when the number of labels are large. However, since \textit{all} and \textit{except} takes longer coding lengths than \textit{add}, they are considered harder to learn. Thus a dataset with only $1\%$ of the labels should be easier to learn than one with $99\%$ of the labels.

% \begin{table}
% \centering
% \begin{tabular}{c|cccccccc}
% \toprule
% \% of labels & 1 & 4 & 16 & 32 & 50 & 84 & 96 & 99 \\\midrule
% AUC & 1.000 & 1.000 & 0.987 & 0.601 & 0.543 & 0.551 & 0.565 & 0.611 \\
% \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{AUC scores for the generated distribution when trained on datasets with different portions of randomly preselected labels. Higher is better.}
% \label{tab:auc}
% \end{table}

% In order to make a fair and quantitative comparison between the performance of generative models trained on different datasets, we consider the AUC score~\citep{bradley1997use}, which is a widely used metric to evaluate the performance of classifiers and is independent of the portion of positive/negative labels. 
% Since we are able to evaluate the probability of each label from the distribution of generated samples, we are able to evaluate the ``confidence'' of the generative model that a label belongs to the true distribution -- labels with higher probability in the generated samples are more likely to occur in the true distribution as suggested by the generative model. Hence, we treat the evaluation of a generative model as the evaluation of a classifier that outputs real values for each label. AUC values range from $0$ to $1$: a score of $1$ is perfect, a score of $0.5$ suggests that the prediction is no better than a random classifier, and a score less than $0.5$ means that the classifier is worse than randomly guessing the labels.

% Table \ref{tab:auc} contains the AUC scores of generated distributions where the model is trained on different datasets. For cases where the portion of labels are small (\textit{and} case), the model is able to generate all the modes and obtain a perfect AUC. However, for cases where the portion is large (\textit{all} + \textit{except} case), the model achieves a much worse AUC even when the portion of exceptions is small. This suggests that it might be much harder for the model to learn ``exceptions'' than learn ``enumerations''. What is also surprising is that the model actually performs better when there are more labels in this case; this seems to be in contrast to the common conception that GANs tend to miss modes when the model does not enough capacity. 

% While this cannot be simply explained by the ``missing modes phenomenon'', all these results can be explained by our hypothesis for the proposed encoding scheme - if the distribution is harder to encode, it is harder for GANs to learn the distribution; as a consequence, GANs will learn some imperfect distribution that it could represent using the coding length that it is provided with. We show more detailed figures in the Appendix.

% \subsection{Learning to Utilize Encoding Capacity}
% In this experiment, we set up the following constraints for the images: the sum of the top two digits equal the value of the digit at the bottom, i.e., $X_3 = X_1 + X_2$. Based on this constraint, we build up a dataset which contains $\sum_{i=1}^{9} i = 55$ possible configurations, which we call Sum3.

% Since this only contains $5.5\%$ of the entire possible labels, it should be easy to learn the distribution with GANs as it can be represented easily with the \textit{add} operation, as shown in Figure \ref{fig:sum3}. We also considered a case in which the distribution contains 51 of the 55 configurations (Sum\texttt{-{}-}), and the model is also able to learn it reasonably well (in Figure \ref{fig:sum--} in the Appendix).

% We visualize the graduate change of label distribution during training the Sum3 dataset and show how the generative model is able to gradually utilize this encoding capacity. Initially (at around 1000 iterations) the dataset appears to exhibit certain repeating patterns, which suggest that $(X_1, X_2)$ and $X_3$ are relatively uncorrelated at this point of training. This is because the \textit{independence of variables} relation is easier to encode than \textit{adding} all the cases, and the model attempts to approximate the true distribution with a factored distribution $p(X_1, X_2)p(X_3)$. Later on (at around 5000 - 9000 iterations), this patten begins to disappear and the model learns to pick out the distributions of $p(X_1, X_2)$ under different $X_3$ values. Finally (at around 25000 - 40000 iterations) the model learn to match the Sum3 dataset reasonably well, placing high probability values on the true labels, and low probability on other regions.


% \begin{figure*}
% \centering
% \subfigure{\includegraphics[width=0.9\textwidth]{img/sum3_1}}
% \vspace{-1em}
% \subfigure{\includegraphics[width=0.9\textwidth]{img/sum3_2}}
% \vspace{-1em}
% \subfigure{\includegraphics[width=0.9\textwidth]{img/sum3_3}}
% \caption{Heat maps of labels of generated distribution trained on the Sum3 dataset.}
% \label{fig:sum3}
% \end{figure*}

% \paragraph{Evaluation.}
% For evaluation, we still use the pretrained MNIST classifier to detect the 3 digits in generated images. GANs begin to generate reasonable images after the first 1,000 iterations, since then, we begin to monitor the combination distribution of the digits in generated images. As is shown in Fig~\ref{Sum3Result}, as the training moves on, the generator gradually learns to encode the certain combinations and decreases the probability of other wrong combinations. The probability on the 9 correct diagonal is higher than other points. However, unlike Num3 experiment, the distribution of the digit on each 3 locations from the Sum3 dataset is not uniform --- digit ``0'' certainly shows up more frequently than digit ``9'' on top two locations. As is shown on the heatmap, although all the correct combinations are more likely to generate, images with digit ``0'' on the top or ``9'' on the bottom still have high probabilities.

% We further eliminate 4 combinations: (1, 8, 9), (4, 5, 9), (0, 6, 6) and (3, 2, 5). Images with the 4 combinations do not show up in the Sum3\texttt{-{}-}. The heat map in Fig~\ref{Sum3Result} shows that GANs have not learned to generate the 4 samples although these 4 can be easily deducted and generalized.

\iffalse
\subsection{InfoDigit}
\paragraph{Dataset.} In this experiment, we further perform experiments on continuous combinations. We design InfoDigit dataset based on a pretrained InfoGAN model~\cite{chen2016infogan}. InfoGAN is capable of disentangling the features by maximizing the mutual information between the input latent codes and the observation. For this experiment, we adopt a InfoGAN model pretrained on MNIST~\cite{lecun2010mnist}, which has 12 dimensional latent codes (10 categorical and 2 continuous). One continuous code varies from -2 to 2, representing the digit rotation. We input latent code -2 (most left leaning) and 2 (most right leaning), and generate images by the generator, thus building up InfoDigit dataset.

\begin{figure*}
\centering
\subfigure{\includegraphics[width=0.3\textwidth]{img/info.pdf}}
~
\subfigure{\includegraphics[width=0.3\textwidth]{img/info_truth}
}
~
\subfigure{\includegraphics[width=0.3\textwidth]{img/info_dist}
}
\caption{Distribution of generated images (left) and dataset (ground truth, middle). They basically match and few interpolation happens. The distribution of generated digits is on the right.
}
\label{InfoResult}
\end{figure*}

\begin{wrapfigure}{R}{0.3\textwidth}
\centering
\includegraphics[width=0.3\textwidth]{img/0158.png}
\caption{\label{fig:infosample}Samples of the generative model that is trained on InfoDigit.}
\end{wrapfigure}

\paragraph{Evaluation.} As is shown in Fig~\ref{InfoResult}, the distribution of InfoDigit is shown in the right image, the outputs of the posterior (classifier) network in the pretrained InfoGAN model cluster around -1.5 and 1.5. After 60,000 iterations of training on InfoDigit, the generative model also learns to generate the images that are either left leaning or right leaning, producing few interpolations, such as no leaning digit. The generative model shows weak generalization in this setting. Some samples are shown in Fig~\ref{fig:infosample}
\fi

%\input{capacity}
\section{Discussion}

We know: discriminator trained by correct combination vs. incorrect combination can correctly distinguish them.

discriminator trained on generated samples vs. correct combination?

generator cannot produce only correct combinations. 

If both generator and discriminator can produce correct combinations (there is a saddle point), then it's a problem with the adversarial training procedure. There are two possibilities:

1. does not reach saddle point. 

2. sinks into a bad saddle point. 


Two possible fixes: 1. add additional classification term. 2. anneal learning rate


\subsection{Old Draft: Digits}
Digits are ubiquitous in human life. Humans are trained to recognize digits from very early age. Neuroscientists have found that specific neuronal populations in the ventral temporal cortex have larger electrophysiological responses to visual numerals compared with control stimuli \cite{arsalidou20112}. Given images that each contains $k$ digits, humans are able to memorize the appeared combinations when only a small amount are shown, and begin to generalize (or forget) when they see many configurations, even repeatedly. \ay{not sure if we have evidence for that} In this experiment, we aim to assess the behavior of the generative models on the same task.

\paragraph{Experiment Setting} Dataset: We build the dataset with images that contain 3 MNIST digits at fixed locations (top left, top right, bottom left, 28$\times$28 each). Thus we have a universal set of combinations with $10^3=1000$ elements. We randomly picked subsets of the 1000 combinations, and construct the datasets for the training of generative models, where the digit combination in each image is in the given subset. Note that each combinations are uniformly distributed in each training dataset.

Evaluation: The combination of each generated sample is obtained by running a pretrained MNIST classifier on the three patches (top left, top right, bottom left) with \hr{num} error, resulting in one prediction for each patch. We then combine the three prediction to obtain 1 out of the 1000 combinations as the predicted combination for the given generated image. 


In the previous sections, we show that the generative models have similar generalization behavior as humans in peephole settings, where only single type of feature is showed to the models. How would the behavior of the generative models be in real-world data with multi-modal features? Psychological research has shown that humans have a sophisticated bias when they are dealing with multiple feature with multiple modes \hr{cite} \ay{need discussion}. First, the difficulty for human visual system to memorize or encode the exact distribution varies from feature to feature, leading to various generalization behaviors when humans observe various features. In this section, we aim to compare the generalization behaviors as well as the memorization capacity of generative models to that of humans given multiple common features. 

\subsubsection{Old Draft: Preference and Memorization between Shape and Color}
Shape and color are two most typical features, how the generative models would behave when they are trained on datasets with different shape$\times$color configurations is certainly of great interest. Given a large set of configurations, where we have $m$ shapes and $k$ colors, humans can often generalize to the universal set even if they have only seen some of the configurations. There have also been psychological studies that show that humans are more sensitive to colors, i.e., compared to shape configurations, color scheme is more likely to be memorized \hr{needs proof} and thus, harder to be generalized. Based on this phenomenon, we conduct experiments with similar setting on generative models. Given the shape$\times$color configuration matrix, we compare the generalization and memorization capacity of the generative models to that of the humans when the models are trained on datasets whose configuration matrix has one sparse row or column.

\paragraph{Experiment Settings} Dataset and Model: we use Clevr dataset for this experiment where each image has 2 objects with a set of configurations of $m$ shapes and $k$ colors. The 2 objects are strictly left-right separated from each other. As illustrated in figure, different ordering of colors and shapes is considered different. So we have a universal set of configurations with $m^2\times{k}^2$ elements. Specifically, the color set is $\{blue, red, green, brown\}$, the shape set is $\{cylinder, cone, sphere, torus\}$, each element in both sets is considered easy enough to be distinguished from another by humans. We use the WGAN-GP for training and evaluation in this experiment with same architecture and hyper-parameters as in previous experiments.

Evaluation: We show the \hr{num} human judges with \hr{num} generated images. The same tests (test on labeled set and test-retest) are still performed to enforce high reliability of the judges. The judges assess and label each image with the configuration. We evaluate the generalization behavior by comparing the \hr{specific} divergence between the generated and the empirical distribution. 

\paragraph{Preliminary Results} For the 81 configurations, unfortunately, the generative model can still memorize the configuration and shows little generalization behavior. There is almost none color generalization, but we can see some (not much) generalization of shapes, although the reason is probably cylinders and cubes are difficult to distinguish. I am enlarging the dataset with 16 color configuration $\times$ 9 shape configurations. Let's hope it works. And then if we have some generalization behavior, we could probably talk about the 100 story, including random noise, shape-color and MNIST, if we still have space.

Besides the surprisingly similar generalization behavior of the generative models and humans on various tasks, we also find that the generative model seems to have a limited memorization capacity, which happens to be 100 configurations in both the digit and shape$\times$color experiments. We further conduct an experiment on random noise to validate the hypothesis in a rather brute-force way. \hr{add random noise exp and some discussion}



%\section{Introduction}


%~\footnote{Another example of this ill-definition is discussed by Pierre-Simon Laplace with the Sunrise problem. Whether the sun rises each day is not an i.i.d sample from some ground truth distribution, nor is it reasonable to place any Bayesian prior on this probability. As a result probability theory have great difficulty discussing such phenomenon.}. 



% This is different from the typical setting of classification. For classification (modeling $p(y|x)$), the ground truth is provided by humans, so there is no discrepency between true distribution $p^*$ and the human distribution $p_m$. (maybe?) However the same is not true for generative models, as they are often collected from natural images, and are not completely human inventions. 

% Answering this question requires human intuition and judgment. A typical example is to traverse the manifold ~\cite{radford2015unsupervised} by constructing a path in the latent feature space from one example to another, and observe how the output varies. A model that generalizes should generate a meaningful sequence of interpolations between the two examples. In addition, each step of the interpolation should agree with human judgment. For example, the existence of white and black flowers and white snow does not imply the existence of black snow, so such an interpolation would be considered ``incorrect'' by human experience. 
% %However, there is no principled measure of such generalization behavior, or related theory.

% This paper attempts to explore this question. We design a synthetic dataset to quantitatively evaluate the generalization behavior of GANs by combining existing real world datasets, e.g., generating images with multiple MNIST digits. %\shengjia{I feel that "the use of labels" is a little confusing}. 
% We train a generative model on a subset of all possible three digit combinations, and observe when GANs generalize to unseen combinations. We observe that the generalization behavior can be explained with the principle of Minimum Description Length~\cite{rissanen1978modeling}. When a generative model can effectively memorize all valid combinations, no generalization will/should occur. Generalization occurs only when a generative model can no longer remember all valid combinations, and it will select an approximating set of label combinations that is easier to represent. 
%Note again that ``generalization'' here neither implies desired nor undesired behavior, but nonetheless we are in a position to discuss and theorize about the empirical behavior of existing models, and compare this behavior with human generalization behavior. 

 %This may be a critical difference between generative and discriminative models, and is potentially the explanation that generative models have trouble capturing high level relationships (such as remembering how many legs each animal has, see ImageNet samples in \cite{salimans2016improved}).


==> removed.tex <==
\section{Inductive Bias of Human Peripheral Vision System}
In the previous section we show that generative models capture many important features identified with the human vision system. In this section, we will investigate the overall match between structure captured by the human peripheral vision system, and the structured captured by GANs. We have two major findings:

\textbf{1)} On natural images (CIFAR, LSUN, Imagenet), even though humans can clearly identify the generated images as fake, when they appear on the side, our peripheral vision cannot distinguish generated images from real images.

\textbf{2)} Furthermore, our peripheral vision system is not only fooled to believe that generated images are real, they are also able to extract meaningful structure from the generated image. For CIFAR we show that humans can classify the samples to the correct class (even for the fake samples), and for LSUN we show that humans can generate fairly accurate descriptions of the scene. 


\subsection{Experiment Setting}
$n$ subjects participated in the two-alternative-forced-choice task to select the real image from two images. Each participants completed 45 trials. After they chose the real image, they were asked to classify the image they selected into one class from ``Aircraft'', ``Automobile'', ``Bird'', ``Cat'' and ``Deer''.  Throughout the stimuli presentation period, there was always a fixation cross at the center of the screen. The vertical positions of the images are the same as the fixation cross and the horizontal positions of the images are $x$ view angels away from the center. To encourage the subjects to fixate on the fixation cross, we randomly inserted 5 catch trials in the experimental trials in which the white fixation cross would suddenly turn to yellow and the participants need to detect as quickly as possible. We use the accuracy of detecting the color change of the fixation cross as a sanity check to make sure that participants use their peripheral vision to process those images. 

\subsection{Results}
On the CIFAR data, we found that the average accuracy of identifying real image is $57\%$, which is not significantly different from chance. The accuracy of classification on generated images is $83.7\%$ and the  accuracy of classification on generated images is $84.2\%$.

\begin{table}
\centering 
\begin{tabular}{cccc}
\includegraphics[width=0.2\linewidth]{img/lsun_fake1} & 
\includegraphics[width=0.2\linewidth]{img/lsun_fake2} &  
\includegraphics[width=0.2\linewidth]{img/lsun_fake3} &
\includegraphics[width=0.2\linewidth]{img/lsun_fake4} \\
\begin{minipage}{0.2\linewidth} Church with two towers and blue sky \end{minipage} & 
\begin{minipage}{0.2\linewidth} Many people in a room \end{minipage} & 
\begin{minipage}{0.2\linewidth} Building with orange walls and lots of windows \end{minipage} &
\begin{minipage}{0.2\linewidth} Room with square surrounding tables and chairs \end{minipage}
\end{tabular}
\vspace{1ex}
\caption{Randomly selected fake images humans mistaken as real, and their generated descriptions. The richness of these descriptions indicate that humans are able to extract a significant amount of structural information from the image, while ignoring less important structure. As a result, humans peripheral vision cannot identify these images as fake, but can identify the content of the image.}
\end{table}

\subsection{Discussion}



==> save.tex <==
%To further investigate the generalization or deduction ability, we eliminate 4 specific combinations from all the Sum3 combinations (which is 55), and set up the Sum3\texttt{-{}-} dataset.


% \section{Experimental Results}
% To investigate the generalization ability of generative models, we design the following experiments: Num3 and InfoDigit. 
% \subsection{Num3}
% \paragraph{Dataset.} In this experiment, we first design Num3 dataset based on MNIST~\cite{lecun2010mnist}. Every image in Num3 dataset contains 3 hand-written digits from MNIST, located on the top left, top right and bottom left corner of the image. It's easily calculated that there are 1,000 combinations of the 3 digits in each image. For this experiment, we randomly pick 1\%, 4\%, 16\%, 32\%, 50\%, 84\%, 96\%, 99\% of the combinations, build up datasets with the images that contain one of the chosen combinations, thus achieving Rand1\%, Rand4\%, \dots , Rand99\% subsets. The distribution of the 10 digits on each location is set to be uniform. Each subset contains 200,000 images, we hereby investigate the output of the generative models trained on each subset. For the convenience of testing, we train a MNIST classifier, on which we rely during testing to detect the combination of the generated samples. 

% \paragraph{Evaluation.} As a preliminary experiment, we first train a classifier with the same structure of the discriminator, which aims to distinguish the images with combination in the dataset from images with an unseen combination. After 1,000 iterations, the classifier can easily do the binary classification task, which lies a foundation for our adversarial training.

% The experimental results are shown in Fig~\ref{Num31} and Fig~\ref{Num32}. GANs can encode the correct distribution of combinations and only generate the images that meet the combination requirement when the correct or unseen combinations are a small proportion of the whole. As the proportion of correct combinations increases to 50\%, GANs find it harder and harder to learn the correct manifold. However, when the correct combinations are over 50\%, GANs only need to ``eliminate'' the combinations that do not belong to the dataset, and thus GANs gradually learns the correct manifold. As is shown in the charts, GANs are able to learn the correct manifold in Rand1\%, Rand4\% and Rand16\%, with the correct combinations (blue points) appearing more frequently than unseen ones (orange points). The combinations are messed up in the Rand32\%, Rand50\% and Rand84\%. The sum of wrong samples becomes smaller in Rand96\% and Rand99\%. AUC (Area Under the Curve)~\cite{bradley1997use} for each dataset are also tested for evaluation, with Rand1\% to Rand99\% achieving 1, 1, 0.987, 0.601, 0.543, 0.551, 0.565, 0.611. We can see a parabola result although when the correct combinations almost fill up the whole, GANs learn to generate many unseen combinations.

% \subsubsection{Sum3 and Sum3\texttt{-{}-}}
% \paragraph{Dataset.} As a special case, we try to see whether generative models have the ability to reason and deduct as humans. In this experiment, we set up the following constraints for the images: the sum of the top two digits equal the value of the digit at the bottom. Based on this constraint, we build up Sum3 dataset. To further investigate the generalization or deduction ability, we eliminate 4 specific combinations from all the Sum3 combinations (which is 55), and set up the Sum3\texttt{-{}-} dataset.
